Mutual-Information Based Few-Shot Classification

We introduce Transductive Infomation Maximization (TIM) for few-shot learning. Our method maximizes the mutual information between the query features and their label predictions for a given few-shot task, in conjunction with a supervision loss based on the support set. We motivate our transductive loss by deriving a formal relation between the classification accuracy and mutual-information maximization. Furthermore, we propose a new alternating-direction solver, which substantially speeds up transductive inference over gradient-based optimization, while yielding competitive accuracy. We also provide a convergence analysis of our solver based on Zangwill's theory and bound-optimization arguments. TIM inference is modular: it can be used on top of any base-training feature extractor. Following standard transductive few-shot settings, our comprehensive experiments demonstrate that TIM outperforms state-of-the-art methods significantly across various datasets and networks, while used on top of a fixed feature extractor trained with simple cross-entropy on the base classes, without resorting to complex meta-learning schemes. It consistently brings between 2 % and 5 % improvement in accuracy over the best performing method, not only on all the well-established few-shot benchmarks but also on more challenging scenarios, with random tasks, domain shift and larger numbers of classes, as in the recently introduced META-DATASET. Our code is publicly available at https://github.com/mboudiaf/TIM. We also publicly release a standalone PyTorch implementation of META-DATASET, along with additional benchmarking results, at https://github.com/mboudiaf/pytorch-meta-dataset.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/bios.tex <==
\clearpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=2in,clip,keepaspectratio]{photos/malik.jpg}}]{Malik Boudiaf} is a PhD candidate at ÉTS Montréal, Canada, supervised by Prof. Ismail Ben Ayed and Prof. Pablo Piantanida. He obtained his MSc in Aeronautics \& Astronautics from Stanford University in 2019, and his M.Eng in Aerospace Engineering from ISAE-Supaero, France in 2017. His current research interests lie between Computer Vision, Information Theory and Optimization, and their application to few-shot/unsupervised learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=2in,clip,keepaspectratio]{photos/ziko.jpg}}]{Imtiaz Masud Ziko} obtained his PhD from \'ETS Montreal, Canada in 2020, supervised by Prof. Ismail Ben Ayed. Currently, He works as a Research Scientist in Thales, Canada. His current research works and interests are around Clustering, Few-shot Learning, Explainable AI and Fairness in Machine learning algorithms.  

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=2in,clip,keepaspectratio]{photos/jerome.jpg}}]{Jérôme Rony} is a PhD candidate at ÉTS Montréal, Canada, supervised by Prof. Ismail Ben Ayed and Prof. Marco Pedersoli. He obtained his M.Eng. in industrial engineering from Arts et Métiers, France in 2018 and his M.A.Sc in system engineering from ÉTS Montréal in 2020. His research interests are in machine learning, computer vision and optimization and their application to adversarial examples and deep learning with constraints.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=2in,clip,keepaspectratio]{photos/Jose_IEEE.png}}]{Jose Dolz} obtained a PhD with the highest honors in Applied Mathematics from the University of Lille 2 in 2016. He was awarded with a Marie-Curie scholarship to pursue his doctoral studies. After that, he was postdoctoral researcher at the \'ETS Montreal, where he is currently Assistant Professor in the Dept. of Software and IT Engineering. His current research interests include medical image analysis, image segmentation, multi-modal learning and weakly supervised learning. Jose serves as regular reviewer for the main conferences and journals in medical imaging, machine learning and computer vision, having been selected as outstanding reviewer in ECCV'20 and \textsc{Miccai}'20. He has also served as Area Chair for \textsc{Midl}'20 and \textsc{Miccai}'21. Furthermore, he has given 2 tutorials in weakly supervised learning at well-known conferences (\textsc{Miccai}'19,\textsc{Miccai}'20).

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=2in,clip,keepaspectratio]{photos/ismail.jpeg}}]{Ismail Ben Ayed} is currently a Full Professor at \'ETS Montreal. He is also affiliated with the CRCHUM. His interests are in computer vision, optimization, machine learning and medical image analysis algorithms. Ismail authored over 100 fully peer-reviewed papers, mostly published in the top venues of those areas, along with 2 books and 7 US patents.  In the recent years, he gave over 30 invited talks, including 4 tutorials at flagship conferences (\textsc{Miccai}'14, \textsc{Isbi}'16, \textsc{Miccai}'19 and \textsc{Miccai}'20). His research has been covered in several visible media outlets, such as Radio Canada (CBC), Quebec Science Magazine and Canal du Savoir. His research team received several recent distinctions, such as the \textsc{Midl}'19 best paper runner-up award and several top-ranking positions in internationally visible contests. Ismail served as Program Committee for \textsc{Miccai}'15, \textsc{Miccai}'17 and \textsc{Miccai}'19, and as Program Chair for \textsc{Midl}'20. Also, he serves regularly as reviewer for the main scientific journals of his field, and was selected several times among the top reviewers of prestigious conferences (such as CVPR'15 and \textsc{NeurIPS}'20).

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=2in,clip,keepaspectratio]{photos/Pablo.jpg}}]{Pablo Piantanida} (Senior Member, IEEE) received the  B.Sc.  degree  in  electrical  engineering  and  the M.Sc. degree from the University of Buenos Aires, Argentina,   in   2003,   and   the   Ph.D.   degree   from Université Paris-Sud, Orsay, France, in 2007. He is currently Professor with the Laboratoire des Signaux et Systèmes (L2S), CentraleSupélec together with CNRS and Université Paris-Saclay. He is also an associate member of Comète – Inria research team (Lix - Ecole Polytechnique) and the Montreal Institute for Learning Algorithms (Mila). His research interests include  information theory, machine learning, security of  learning systems and the secure processing of information and applications to computer vision, health, natural language processing, among others. He has served as the General Co-Chair for the 2019 \textit{IEEE  International  Symposium  on  Information  Theory  (ISIT)}.  He  serves  as an  Associate  Editor  for  the  \textit{IEEE  Transactions  On  Information Forensics And Security} and Editorial Board of Section ``Information Theory, Probability and Statistics'' for Entropy. He is member of the IEEE Information Theory Society Conference Committee.
\end{IEEEbiography}



